Towards Robust Multimodal Learning in the Open World

The rapid evolution of machine learning has propelled neural networks to unprecedented success across diverse domains. In particular, multimodal learning has emerged as a transformative paradigm, leveraging complementary information from heterogeneous data streams (e.g., text, vision, audio) to advance contextual reasoning and intelligent decision-making. Despite these advancements, current neural network-based models often fall short in open-world environments characterized by inherent unpredictability, where unpredictable environmental composition dynamics, incomplete modality inputs, and spurious distributions relations critically undermine system reliability. While humans naturally adapt to such dynamic, ambiguous scenarios, artificial intelligence systems exhibit stark limitations in robustness, particularly when processing multimodal signals under real-world complexity. This study investigates the fundamental challenge of multimodal learning robustness in open-world settings, aiming to bridge the gap between controlled experimental performance and practical deployment requirements.

==> Chapter_7.tex <==
% % Chapter 7

% \chapter{List of Publications}

% \label{Chapter7}

% \section{Published}

% \begin{enumerate}
%     \item \textbf{Zicong Hong}, Song Guo, Rui Zhang, Peng Li, Yufeng Zhan, and Wuhui Chen, "CYCLE: Sustainable Off-Chain Payment Channel Network with Asynchronous Rebalancing", accepted by the 52nd Annual IEEE/IFIP International Conference on Dependable Systems and Networks (DSN) (CCF-B), 2022.
%     \item \textbf{Zicong Hong}, Song Guo, and Peng Li, "Scaling Blockchain via Layered Sharding", accepted by IEEE Journal on Selected Areas in Communications (JSAC) (CCF-A), 2022.
%     \item \textbf{Zicong Hong}, Song Guo, Peng Li, and Wuhui Chen, "Pyramid: A Layered Sharding Blockchain System", accepted by IEEE International Conference on Computer Communications (INFOCOM) (CCF-A), 2021.
%     \item Jianting Zhang*, \textbf{Zicong Hong}*, Yufen Zhan, Song Guo, and Wuhui Chen, "SkyChain: A Deep Reinforcement Learning-Empowered Dynamic Sharding Blockchain System", accepted by International Conference on Parallel Processing (ICPP) (Best paper runner-up price, CCF-B), 2020 (*The first two authors have equal contribution).
%     \item Ting Cai, \textbf{Zicong Hong}, Shuo Liu, Wuhui Chen, Zibin Zheng, and Yang Yu, "SocialChain: Decoupling Social Data and Applications to Return Your Data Ownership", accepted by IEEE Transactions on Services Computing (TSC) (CCF-B, JCR Q1), 2021
%     \item Leijie Wu, Song Guo, Yi Liu, \textbf{Zicong Hong}, Yufen Zhan and Wenchao Xu, "Sustainable Federated Learning with Long-term Online VCG Auction Mechanism", accepted by International Conference on Distributed Computing Systems (ICDCS) (CCF-B), 2022.
%     \item Yi Liu, Leijie Wu, Yufeng Zhan, Song Guo, and \textbf{Zicong Hong}, "Incentive-Driven Long-term Optimization for Edge Learning by Hierarchical Reinforcement Mechanism", accepted by International Conference on Distributed Computing Systems (ICDCS) (CCF-B), 2021.
%     \item Yufeng Zhan, Jie Zhang, \textbf{Zicong Hong}, Leijie Wu, Peng Li, and Song Guo, "A Survey of Incentive Mechanism Design for Federated Learning", accepted by IEEE Transactions on Emerging Topics in Computing (TETC) (JCR Q1), 2021.
% \end{enumerate}

% \section{Under Review}

% \begin{enumerate}
%     \item Enyuan Zhou, \textbf{Zicong Hong}, Yang Xiao, Dongxiao Zhao, Qingqi Pei, Song Guo and Rajendra Akerkar, "MSTDB: A Hybrid Storage-empowered Scalable Semantic Blockchain Database", under the major revision of IEEE Transactions on Knowledge and Data Engineering (TKDE) (CCF-A).
%     \item Jianting Zhang, \textbf{Zicong Hong}, Xiaoyu Qiu, Wuhui Chen, Yufeng Zhan and Song Guo, "Scaling Blockchain via Dynamic Sharding", revise and resubmit as New for IEEE Transactions on Dependable and Secure Computing (TDSC) (CCF-A).
%     \item \textbf{Zicong Hong}, Song Guo, Enyuan Zhou, Jianting Zhang, Wuhui Chen and Jinwen Liang, "Prophet: A Sharding Blockchain System with Deterministic Ordering for Conflict-Free Transactions", submitted to USENIX Symposium on Networked Systems Design and Implementation (NSDI) (CCF-A).
%     \item \textbf{Zicong Hong}, Song Guo, Enyuan Zhou, Wuhui Chen, Huawei Huang and Albert Zomaya, "GriDB: Scalable Blockchain Database via Off Chain-Empowered Sharding", submitted to IEEE International Conference on Data Engineering (ICDE) (CCF-A).
%     \item Enyuan Zhou, Song Guo, \textbf{Zicong Hong}, Jinwen Liang, Jingyi Tian, Peixin Yue and Qingqi Pei, "VeriKG: Hybrid Knowledge Graph Blockchain with Verifiable SPARQL", submitted to IEEE International Conference on Data Engineering (ICDE) (CCF-A).
%     \item Jianting Zhang, Wuhui Chen, \textbf{Zicong Hong}, Gang Xiao, Linlin Du and Zibin Zheng, "Efficient Execution of Arbitrarily Complex Cross-shard Contracts for Blockchain Sharding", submitted to IEEE Transactions on Knowledge and Data Engineering (TKDE) (CCF-A).
%     \item Leijie Wu, Song Guo, Junxiao Wang, \textbf{Zicong Hong}, Jie Zhang and Yaohong Ding, "Federated Unlearning: Guarantee the Right of Clients to Forget", submitted to IEEE Network Magazine (JCR Q1).
%     \item Wuhui Chen, Xiaoyu Qiu, \textbf{Zicong Hong}, Zibin Zheng, Hong-Ning Dai and Jianting Zhang, "Proactive Look-Ahead Control of Transaction Flows for High-Throughput Payment Channel Network", submitted to ACM Symposium on Cloud Computing (SoCC) (CCF-B).
%     \item Zhongteng Cai, Junyuan Liang, Wuhui Chen, \textbf{Zicong Hong}, Hong-Ning Dai, Jianting Zhang and Zibin Zheng, "Benzene: Scaling Blockchain with Cooperation-Based Sharding", submitted to IEEE Transactions on Parallel and Distributed Systems (TPDS) (CCF-A).
% \end{enumerate}
